Monochromatic Triangles, Triangle Listing and APSP

One of the main hypotheses in fine-grained complexity is that All-Pairs Shortest Paths (APSP) for $n$-node graphs requires $n^{3-o(1)}$ time. Another famous hypothesis is that the $3$SUM problem for $n$ integers requires $n^{2-o(1)}$ time. Although there are no direct reductions between $3$SUM and APSP, it is known that they are related: there is a problem, $(\min,+)$-convolution that reduces in a fine-grained way to both, and a problem Exact Triangle that both fine-grained reduce to. In this paper we find more relationships between these two problems and other basic problems. P\u{a}tra\c{s}cu had shown that under the $3$SUM hypothesis the All-Edges Sparse Triangle problem in $m$-edge graphs requires $m^{4/3-o(1)}$ time. The latter problem asks to determine for every edge $e$, whether $e$ is in a triangle. It is equivalent to the problem of listing $m$ triangles in an $m$-edge graph where $m=\tilde{O}(n^{1.5})$, and can be solved in $O(m^{1.41})$ time [Alon et al.'97] with the current matrix multiplication bounds, and in $\tilde{O}(m^{4/3})$ time if $\omega=2$. We show that one can reduce Exact Triangle to All-Edges Sparse Triangle, showing that All-Edges Sparse Triangle (and hence Triangle Listing) requires $m^{4/3-o(1)}$ time also assuming the APSP hypothesis. This allows us to provide APSP-hardness for many dynamic problems that were previously known to be hard under the $3$SUM hypothesis. We also consider the previously studied All-Edges Monochromatic Triangle problem. Via work of [Lincoln et al.'20], our result on All-Edges Sparse Triangle implies that if the All-Edges Monochromatic Triangle problem has an $O(n^{2.5-\epsilon})$ time algorithm for $\epsilon>0$, then both the APSP and $3$SUM hypotheses are false. We also connect the problem to other ``intermediate'' problems, whose runtimes are between $O(n^\omega)$ and $O(n^3)$, such as the Max-Min product problem.

==> non_reducibility.tex <==
We showed reduction from Exact Triangle to triangle listing problems, which imply that such triangle listing problems are hard under both APSP and $3$SUM. Thus, it is natural to ask if we can reduce from the other famous conjecture in find-grained complexity -- Strong Exponential Time Hypothesis (SETH) -- to such triangle listing problems.

As shown in \cite{carmosino2016nondeterministic}, if we could show $T(n)$ time nondeterminisitc/co-nondeterminisitc algoirthms for a problem $P$, then \textit{deterministic} reduction from SETH cannot show lower bound greater than $T(n)$, assuming the Nondeterministic Strong Exponential Time Hypothesis (NSETH) conjecture. 


\begin{proposition}
\label{prop:non_reduce}
Fix any constants $\alpha, \beta, \gamma > 0, \rho < \min\{\alpha, \beta, \gamma\}$ and a sufficiently large constant $C$. 
Let $$t = \min_{0 \le x \le \alpha, 0 \le y \le \beta, 0 \le z \le \gamma} \max\left\{2\alpha + 2\beta + 2\gamma - 3\rho - x - y -z, \omega(x, y, z) \}\right\}.$$
Assuming the NSETH conjecture, $(\alpha, \beta, \gamma, \rho, C n^{\alpha + \beta + \gamma - 3\rho})$  Triangle Listing for $T(n) = n^{t + \epsilon}$ is not SETH-hard for any $\epsilon > 0$ (via deterministic reductions). 

\end{proposition}


By Theorem~\ref{thm:exact-to-general-triangle-listing},  $(\alpha, \beta, \gamma, \rho, O(n^{\alpha + \beta + \gamma - 3\rho}))$  Triangle Listing has an   $n^{\alpha + \beta + \gamma - 2\rho - o(1)}$ lower bound assuming Exact Triangle. On the other hand, we can enumerate for all $a \in A$ all pairs of its neighbors in $O(n^{\alpha+\beta-\rho + \gamma - \rho}) = O(n^{\alpha + \beta + \gamma - 2\rho})$ time, so the lower bound from Exact Triangle is tight. Yet Proposition~\ref{prop:non_reduce} shows that we cannot achieve high lower bounds from SETH to it. 

Let's look at a special case for Triangle Listing, when $\alpha = \beta = \gamma = 1$ and $\rho = 0.5$. In this case, we are given an $n$-vertex graph where each vertex has degree bounded by $\sqrt{n}$, and we are asked to list $O(n^{1.5})$ triangles in this graph. 
We simply let $x= y= z$, in which case $t$ becomes $\min_{0 \le x \le 1} \max\{4.5-3x, x\omega\}$. With the current value of $\omega \le 2.373$, $t \le 1.988$, which means there is no tight deterministic reduction from SETH to  $(1, 1, 1, 0.5, O(n^{1.5}))$ Triangle Listing assuming NSETH. If $\omega = 2$, $t = 1.8$ so we get an even better result. 



\begin{proof}[Proof of Proposition~\ref{prop:non_reduce}]
First, we need a notion of nondeterministic algorithms for a problem like triangle listing for which there are multiple output bits. A nondeterministic algorithm is given an input, and an advice string. Based on the advice string, the algorithm could REJECT, in which case there is no constraint on what the algorithm outputs. If the algorithm does not REJECT, it should output the correct answer for the input. For any input, there must be at least one advice string that makes the algorithm output the correct answer. 
Using the framework of \cite{carmosino2016nondeterministic}, it suffices to show an $O(n^t)$ time nondeterministic algorithm for  $(\alpha, \beta, \gamma, \rho, Cn^{\alpha + \beta + \gamma - 3\rho})$ Triangle Listing.

We describe the advice string first. First, the advice string lists up to $Cn^{\alpha + \beta + \gamma - 3\rho}$ triangles in the graph. The algorithm reads these triangles,  tests if they are indeed triangles in the graph. If so, the algorithm could list these triangles as output. If the advice string lists duplicated triangles or non-triangle in the graph, the algorithm REJECTs. 
The only case when the algorithm could be wrong is when the advice string lists $T < Cn^{\alpha + \beta + \gamma - 3\rho}$ triangles, but there are more than $T$ triangles in the graph. Thus, the algorithm needs to verify that the graph only has $T$ triangles for some $T < Cn^{\alpha + \beta + \gamma - 3\rho}$.

To do so, the advice string provides maps $\pi_A: A \mapsto [n^x]$, $\pi_B: B \mapsto [n^y]$, $\pi_C: C \mapsto [n^z]$ for some $x, y, z$ that minimizes the formula for $t$. We consider a multi-graph $G$ on vertex sets $[n^x] \sqcup [n^y] \sqcup [n^z]$. For any edge $(i, j) \in E \cap (A \times B)$, we add an edge $(\pi_A(i), \pi_B(j))$ to $G'$. Similarly, for $(i, k) \in E \cap (A \times C)$, we add an edge $(\pi_A(i), \pi_C(k))$, and for $(j, k) \in E \cap (B \times C)$, we add an edge $(\pi_B(j), \pi_C(k))$. The advice string could provide all triangles in the graph $G'$. If the number of triangles is greater than $O(n^{2\alpha + 2\beta + 2\gamma -3\rho - x - y - z})$, the algorithm REJECTs. Otherwise, the algorithm counts the number of triangles in $G'$ via rectangular matrix multiplication in $O(n^{\omega(x, y, z)})$ time. If the number of triangles computed does not match the number of triangles given by the advice string, the algorithm REJECTs. Otherwise, the algorithm reads all triangles with edges $(e_1, e_2, e_3)$ in $G'$ from the advice string, and tests the corresponding edges of $e_1, e_2, e_3$ in the original graph is one of the $T$ triangles listed. If they do not correspond any of the $T$ triangles, the algorithm has found more than $T$ triangles in the graph, and it REJECTs. If the algorithm does not REJECT, it means that there are indeed only $T$ triangles in the graph, so it is correct to listing these triangles. 


It remains to show that there exists maps $\pi_A, \pi_B, \pi_C$ such that the number of triangles in $G'$ is bounded by $O(n^{2\alpha + 2\beta + 0.5\gamma - x - y - z})$. To do so, we consider random maps $\pi_A: A \mapsto [n^x]$, $\pi_B: B \mapsto [n^y]$, $\pi_C: C \mapsto [n^z]$ and bound the expected number of triangles in $G'$. 

Let $\rho = \gamma / 2$ be density parameter of $G$. 
There are three cases to consider:
\begin{enumerate}
    \item Triangles in $G'$ corresponding to three edges in $G$ that do not share any vertices. In this case, the numbers of triples of edges is $n^{2\alpha +2\beta + 2\gamma- 3\rho}$. Each triple has an $n^{-x-y-z}$ probability to form a triangle. Thus, the expected number of triangles is bounded by $n^{2\alpha +2\beta + 2\gamma- 3\rho - x - y - z}$. We will show this is the dominating case. 
    \item Triangles in $G'$ corresponding to three edges in $G$ that share exactly one vertex. First we assume this vertex $c$ is in $C$. The number of such vertices  is $n^\gamma$. Such a triangle in $G'$ contains two neighboring edges $(c, a)$ and $(c, b)$, and one arbitrary edge $(a', b')$ in $A \times B$. Thus, the total number of choices is $n^{2\alpha + 2\beta + \gamma - 3\rho}$. For each choice, the probability they form a triangle is the probability that $\pi_A(a)=\pi_A(a')$ and $\pi_B(b) = \pi_B(b')$, which happens with probability $n^{-x-y}$. Thus, the expected number of triangles is bounded by $n^{2\alpha + 2\beta + \gamma - 3\rho -x  - y}$, which is dominated by the number triangles in Case 1 since $\gamma \ge z$. Similarly, the cases when the shared vertex is in $A$ or $B$ are also dominated. 
    \item Triangles in $G'$ corresponding to three edges in $G$ that share exactly two vertices. First we assume these two vertices are $(a, b) \in A \times B$. The number of such pairs  is $n^{\alpha+\beta-\rho}$. The other two edges correspond to $(a, c)$ and $(b, c')$ for some $c, c' \in C$. The number of choices $a, b, c, c'$ is $n^{\alpha+\beta+2\gamma - 3\rho}$. Each choice has an $n^{-z}$ probability to actually form a triangle in $G'$, so the expected number of triangles is $n^{\alpha+\beta+2\gamma - 3\rho - z} \le n^{2\alpha +2\beta + 2\gamma- 3\rho - x - y - z}$. By symmetry, the cases when the shared edge is between two other vertex sets are also dominated by Case (1). 
    \item Triangles in $G'$ corresponding to three edges in $G$ that share exactly three vertices. There can be at most $T \le
    Cn^{\alpha + \beta + \gamma - 3\rho}$ of them, which is again dominated by Case (1). 
\end{enumerate}
Since the expected number of triangle is $O(n^{2\alpha +2\beta + 2\gamma- 3\rho - x - y - z})$, there exists $\pi_A, \pi_B, \pi_C$ so that the number of triangles in $G'$ is $O(n^{2\alpha +2\beta + 2\gamma- 3\rho - x - y - z})$.
\end{proof}


Unfortunately, Proposition~\ref{prop:non_reduce} does not always show non-reducibility result for arbitrary choices of parameters of the triangle listing problem. One case is that when the degrees of all vertex are very small, even the above nondeterminisitic algorithm does not beat the brute-force algorithm, even when $\omega = 2$.  
% However, in some interesting cases, Proposition~\ref{prop:non_reduce} does always show non-reducibility when $\omega = 2$. One example case is  when $\alpha+\beta+\gamma-3\rho = \alpha + \beta - \rho$, we need to list $O(1)$ triangles for each edge in $A \times B$ on average, as shown in the following theorem. 

% \begin{claim}
% For any constants $\alpha, \beta, \gamma> 0, 0 < \rho < \min\{\alpha, \beta, \gamma\}$, if $\alpha+\beta+\gamma-3\rho = \alpha + \beta - \rho$, then
% $$\min_{0 \le x \le \alpha, 0 \le y \le \beta, 0 \le z \le \gamma} \max\left\{2\alpha + 2\beta + 2\gamma - 3\rho - x - y -z, x + y + z - \min\{x, y, z\} \right\} < \alpha + \beta + \gamma - 2\rho.$$
% \end{claim}
% \begin{proof}

% The condition $\alpha+\beta+\gamma-3\rho = \alpha + \beta - \rho$ translates to $\gamma = 2\rho$.

% Consider two cases.
% \begin{enumerate}
%     \item $\gamma \le \min\{\alpha, \beta\}$. In this case, we can simply set $x = (1-\epsilon)\alpha, y = (1-\epsilon)\beta, z = (1-\epsilon)\gamma$. It is easy to check $\epsilon$ works if and only if $\epsilon < \frac{0.5 \gamma}{\alpha+\beta + \gamma}$, so such $\epsilon > 0$ exists. 
%     \item $\gamma > \min\{\alpha, \beta\}$. Without loss of generality, assume $\alpha \le \beta$. We set $x = \alpha, y=\beta$ and require that $z \ge \alpha$.
% \end{enumerate}

% Let $\epsilon = \min\{2\min\{\alpha, \beta\} - \gamma, \alpha, \beta\} > 0$. Let $x = \alpha - \epsilon / 6, y = \beta - \epsilon / 6$ and $z = \min\{\alpha, \beta\}$. 

% Then $2\alpha + 2\beta + 2\gamma -3\rho - x - y -z = \alpha+ \beta + (0.5 \gamma - \min\{\alpha, \beta\}) + \epsilon / 3 \le \alpha + \beta - \epsilon / 2 + \epsilon / 3 < \alpha + \beta$. Also, $x+y+z - \min\{x, y, z\} = \alpha + \beta - \epsilon / 3 + \min\{\alpha, \beta\} - \min\{\alpha - \epsilon / 6, \beta -\epsilon / 6, \min\{\alpha, \beta\}\}$. Since $\min\{\alpha - \epsilon / 6, \beta -\epsilon / 6, \min\{\alpha, \beta\}\} \ge \min\{\alpha, \beta\} - \epsilon / 6$, we have that $x+y+z - \min\{x, y, z\} \le \alpha + \beta - \epsilon / 6 < \alpha + \beta$. 




% \end{proof}
